Towards Meaningful Anomaly Detection: The Effect of Counterfactual Explanations on the Investigation of Anomalies in Multivariate Time Series

Detecting rare events is essential in various fields, e.g., in cyber security or maintenance. Often, human experts are supported by anomaly detection systems as continuously monitoring the data is an error-prone and tedious task. However, among the anomalies detected may be events that are rare, e.g., a planned shutdown of a machine, but are not the actual event of interest, e.g., breakdowns of a machine. Therefore, human experts are needed to validate whether the detected anomalies are relevant. We propose to support this anomaly investigation by providing explanations of anomaly detection. Related work only focuses on the technical implementation of explainable anomaly detection and neglects the subsequent human anomaly investigation. To address this research gap, we conduct a behavioral experiment using records of taxi rides in New York City as a testbed. Participants are asked to differentiate extreme weather events from other anomalous events such as holidays or sporting events. Our results show that providing counterfactual explanations do improve the investigation of anomalies, indicating potential for explainable anomaly detection in general.

==> Tables/SLR.tex <==
\begin{sidewaystable}
%\footnotesize
\sidewaystablefn%
\begin{center}
\begin{minipage}{\textheight}
\caption{Results of the structured literature review}
\label{table:slr}
\begin{tabularx}{\textheight}{lccccc}
\hline
\textbf{Ref} & \textbf{Data} & \textbf{Anomaly type}  & \textbf{Model} & \textbf{XAI Technique} \\ 
\hline
\hline
\cite{alfeo_using_2020} & Multivariate & Collective & Dense auto-encoder & Reconstruction Error\\
\hline
\cite{de_candido_interpretable_2021} & Multivariate & Collective & CNN auto-encoder & Reconstruction Error \\
\hline
\cite{dix_three-step_2021} & Multivariate & Collective & Dense auto-encoder & Reconstruction Error \\ 
\hline
\cite{ghalehtaki_unsupervised_2022} & Multivariate & Collective &  LSTM auto-encoder & Reconstruction Error \\
\hline
\cite{agarwal_explainability_2021} & Multivariate & Collective & DDSAE-NN & Feature Importance \\
\hline
\cite{jakubowski_explainable_2021} & Multivariate & Collective &  Quasi-LSTM auto-encoder & Feature Importance\\
\hline
\cite{serradilla_adaptable_2021} & Multivariate & Collective &  2D-CNN auto-encoder & Feature Importance\\
\hline
\cite{tripathy_explaining_2022}& Multivariate & Collective & auto-encoder & Feature Importance \\
\hline
\cite{weldezgina_asres_unsupervised_2021} & Multivariate & Collective &  CGVAE & Feature Importance\\
\hline
\cite{yong_coalitional_2022} & Multivariate & Collective &  Coalitional BAE & Feature Importance\\
\hline
\cite{ameli_unsupervised_2022} & Multivariate & Collective &  LSTM auto-encoder & Feature Importance\\
\hline
\cite{ha_explainable_2022} & Multivariate & Collective &  LSTM auto-encoder & Feature Importance \\
\hline
\cite{holly_autoencoder_2022} & Multivariate & Collective &  LSTM auto-encoder & Feature Importance\\
\hline
\cite{jang_anomaly_2019} & Multivariate & Collective & Dense auto-encoder & Feature Importance\\
\hline
\cite{rad_explainable_2021} & Multivariate & Collective &  Custom & Feature Importance \\
\hline
\cite{hussain_explainable_2022} & Multivariate & Collective & LSTM auto-encoder & Feature Importance\\
\hline
\cite{oliveira_new_2022} & Multivariate & Collective & Dense auto-encoder & Feature Importance\\
\hline
\cite{roelofs_autoencoder-based_2021} & Multivariate & Collective & Dense auto-encoder & Feature Importance \\
\hline
\cite{sulem_diverse_2022} & Multivariate & Collective & LSTM auto-encoder & Counterfactual\\
\hline
\cite{kieu_robust_2022} & Multivariate & Collective & RDAE & Custom \\
\hline
\hline
\end{tabularx}

\end{minipage}
\end{center}
\end{sidewaystable}
